Measurement of four-jet differential cross sections in $\sqrt{s}=8$ TeV proton-proton collisions using the ATLAS detector

Differential cross sections for the production of at least four jets have been measured in proton-proton collisions at $\sqrt{s} = 8$ TeV at the Large Hadron Collider using the ATLAS detector. Events are selected if the four anti-$k_{t}$ R=0.4 jets with the largest transverse momentum ($p_{T}$) within the rapidity range $|y|<2.8$ are well separated ($dR^{\rm min}_{4j}>0.65$), all have $p_{T}>64$ GeV, and include at least one jet with $p_{T} >100$ GeV. The dataset corresponds to an integrated luminosity of 20.3 $fb^{-1}$. The cross sections, corrected for detector effects, are compared to leading-order and next-to-leading-order calculations as a function of the jet momenta, invariant masses, minimum and maximum opening angles and other kinematic variables.

==> tex/acknowledgements.tex <==
We thank CERN for the very successful operation of the LHC, as well as the
support staff from our institutions without whom ATLAS could not be
operated efficiently.

We acknowledge the support of ANPCyT, Argentina; YerPhI, Armenia; ARC,
Australia; BMWF and FWF, Austria; ANAS, Azerbaijan; SSTC, Belarus; CNPq and FAPESP,
Brazil; NSERC, NRC and CFI, Canada; CERN; CONICYT, Chile; CAS, MOST and NSFC,
China; COLCIENCIAS, Colombia; MSMT CR, MPO CR and VSC CR, Czech Republic;
DNRF, DNSRC and Lundbeck Foundation, Denmark; EPLANET, ERC and NSRF, European Union;
IN2P3-CNRS, CEA-DSM/IRFU, France; GNSF, Georgia; BMBF, DFG, HGF, MPG and AvH
Foundation, Germany; GSRT and NSRF, Greece; ISF, MINERVA, GIF, DIP and Benoziyo Center,
Israel; INFN, Italy; MEXT and JSPS, Japan; CNRST, Morocco; FOM and NWO,
Netherlands; BRF and RCN, Norway; MNiSW, Poland; GRICES and FCT, Portugal; MERYS
(MECTS), Romania; MES of Russia and ROSATOM, Russian Federation; JINR; MSTD,
Serbia; MSSR, Slovakia; ARRS and MIZ\v{S}, Slovenia; DST/NRF, South Africa;
MICINN, Spain; SRC and Wallenberg Foundation, Sweden; SER, SNSF and Cantons of
Bern and Geneva, Switzerland; NSC, Taiwan; TAEK, Turkey; STFC, the Royal
Society and Leverhulme Trust, United Kingdom; DOE and NSF, United States of
America.

The crucial computing support from all WLCG partners is acknowledged
gratefully, in particular from CERN and the ATLAS Tier-1 facilities at
TRIUMF (Canada), NDGF (Denmark, Norway, Sweden), CC-IN2P3 (France),
KIT/GridKA (Germany), INFN-CNAF (Italy), NL-T1 (Netherlands), PIC (Spain),
ASGC (Taiwan), RAL (UK) and BNL (USA) and in the Tier-2 facilities
worldwide.


==> tex/triggertable.tex <==
\begin{table*}
\renewcommand\arraystretch{1.5}
\centering
\begin{tabular}{c  c  c ccc  l}
\hline
      & $N_{\mathrm jet}$ & \ptminnom~[GeV] & \multicolumn{3}{c}{Domain of use} & $\int \mathcal{L} \,{\mathrm d}t$ \\
\hline
 \rA: & $\geq$4 & 45  & \SI{100}{\GeV} < ${\pt}_1$ < \SI{320}{\GeV} &and& \SI{64}{\GeV} < ${\pt}_4$ < \SI{76}{\GeV} & \SI{95.2}{\per\pb} \\
 \rB: & $\geq$4 & 65  & \SI{100}{\GeV} < ${\pt}_1$ < \SI{320}{\GeV} &and& \SI{76}{\GeV} < ${\pt}_4$ & \SI{17.4}{\per\fb} \\
 \rC: & $\geq$1 & 280 & \SI{320}{\GeV} < ${\pt}_1$ < \SI{410}{\GeV} &and& \SI{64}{\GeV} < ${\pt}_4$ &   \SI{17.4}{\per\pb}  \\
 \rD: & $\geq$1 & 360 & \SI{410}{\GeV} < ${\pt}_1$ &and& \SI{64}{\GeV} < ${\pt}_4$ &  \SI{20.3}{\per\fb} \\
\hline
\end{tabular}
\caption{\label{tab:trigger}
The table shows the four different jet triggers used. Different jet multiplicity requirements ($N_{\mathrm jet}$) and nominal thresholds \ptminnom{} are used. Each trigger is used in a particular (non-overlapping) domain.  
Only a fraction of events satisfying three of the four triggers were recorded (i.e. these triggers were ``pre-scaled'') to reduce trigger rate, and hence these triggers correspond to a smaller integrated luminosity.
Note that the four jets are required to have $|y|<2.8$ and to be separated 
from one another by at $\dRmin>0.65$.
}
\end{table*}



==> tex/variables.tex <==
\begin{table*}
\centering
\renewcommand\arraystretch{1.7}
\begin{tabular}{c c l}
\hline
Name & Definition & Comment \\
\hline
${\pt}^i$    & Transverse momentum of the $i$th jet & Sorted descending in \pt \\
\HT          & $\sum\limits_{i=1}^{4} {\pt}_i$ &Scalar sum of the \pt of the four jets \\
\mjjjj\       & $\left(\sum\limits_{i=1}^4 E_i\right)^2 - \left(\sum\limits_{i=1}^4 \mathbf{p}_i\right)^2$ & Invariant mass of the four jets \\
\mjjminvar\   & $\min_{\substack{{i,j} \in [1,4] \\ i \neq j}} \left(\left( E_i + E_j \right)^2 - \left( \mathbf{p}_i + \mathbf{p}_j \right)^2\right)$  &  Minimum invariant mass of any two jets \\
\minDphiij\   & $\min_{\substack{i,j \in [1,4]\\i \neq j}}\left(|\phi_i-\phi_j|\right)$ & Min azimuthal separation of two jets \\
\minDrapij\   &  $\min_{\substack{i,j \in [1,4]\\i \neq j}}\left(|y_i-y_j|\right)$ & Min rapidity separation of two jets \\
\minDphiijk\  & $\min_{\substack{i,j,k \in [1,4]\\i \neq j \neq k}}\left(|\Delta\phi_{ij}|+|\Delta\phi_{jk}|\right)$ & Min azimuthal separation between any three jets \\
\minDrapijk\  &  $\min_{\substack{i,j,k \in [1,4]\\i \neq j \neq k}}\left(|\Delta y_{ij}|+|\Delta y_{jk}|\right)$ & Min rapidity separation between  any three jets \\
\maxDrapij\   & $\Delta y^{\max}_{ij} = \max_{i,j \in [1,4]}\left(| y_{i}- y_{j}|\right)$ & Max rapidity difference between two jets \\
\sumptcent\   & Sum of \pt{} of the two central-rapidity jets & Excludes jets having \maxDrapij\ \\
\hline
\end{tabular}
\caption{\label{tab:variables}
Definitions of the various kinematic variables used. Only the four 
jets with the largest \pt{} value are considered. 
}
\end{table*}

Cross sections are measured differentially using the kinematical variables defined in \tabref{tab:variables}.
As well as basic kinematic quantities, such as jet transverse momenta (\pt) and rapidity ($y$) , other variables are selected 
in part to provide sensitivity to differences between different MC models of QCD processes.
For example, the four-jet invariant mass \mjjjj\ is sensitive to the 
largest energy scales in the event whereas \mjjminvar{} probes the smallest jet-splitting scale.
The ratio $\mjjminvar/\mjjjj$ therefore provides information about the range of energy scales relevant to the
QCD calculation.
The variables \maxDrapij\ and \sumptcent\ are designed to be sensitive to events with forward jets.
The azimuthal variable  \minDphiijk{} distinguishes events with pairs of nearby jets 
(with large \minDphiijk) from the recoil of three jets against one (leading to small \minDphiijk\ values).

Distributions of example variables can be seen at the detector level
(i.e. prior to unfolding detector effects) in 
\figref{fig:control_plots}.



